Foundation Models as Modular Tools for fMRI Analysis

Foundation models (FMs) for the brain are rapidly growing in number and each captures a different aspect of the same data. A single scientific question often needs several of them at once, alongside classical analysis and the literature, but no established method combines them, because each model defines its own inputs, outputs, and spatial conventions. Representation alignment, the usual route from an FM into a language model, binds one FM to one LLM and requires retraining for every model added. We take a modular route: each FM becomes an independent tool server that a fixed language agent calls next to classical and literature tools, with no retraining. We start with fMRI, where public FMs already disagree on how to name a brain location and open task data give a classical baseline, and serve two FMs at opposite ends of that spectrum, BrainLM (atlas parcels) and Omni-fMRI (atlas-free voxels). A 76-question benchmark, a 2 by 2 tool ablation, and an independent LLM judge yield 3,040 judged traces. In this first study, modular FM access raises holistic answer quality by $+0.70$ on a 1 to 5 rubric (95% CI $[+0.44, +0.97]$, $n=34$). The gain lands in how the agent selects, parameterizes, and grounds tool calls, and peaks where the agent must cross FM vocabularies. The two FMs win on different questions, yet mounting both matches the better one, and the voxel interface fails 7.8 times more often by context overflow. Modular connection works. Orchestrating what it connects, across EEG and MRI models, is the work ahead.

==> tables_v2/T1_condition_server_matrix.tex <==
\begin{table}[H]
\centering
\caption{Tool-server exposure by condition. piop1 (classical atlas analysis) and pubmed (literature) are always on; the two fMRI foundation-model servers are ablated.}
\label{tab:condition_server_matrix}
\begin{tabular}{lrrrr}
\toprule
condition & piop1 & pubmed & brainlm & omni\_fmri \\
\midrule
classical & on & on & -- & -- \\
brainlm\_only & on & on & on & -- \\
omni\_only & on & on & -- & on \\
full & on & on & on & on \\
\bottomrule
\end{tabular}
\end{table}


==> tables_v2/T2_scope_decision.tex <==
\begin{table}[t]
\centering
\caption{Question families and their scope decisions.}
\label{tab:scope_decision}
\begin{tabular}{lrrrrrrp{6.2cm}}
\toprule
family & n & pooled\_abs\_mean\_holistic & mean\_delta\_full\_minus\_classical & delta\_min & delta\_max & in\_core & reason \\
\midrule
VC & 14 & 3.460 & 1.038 & 0.200 & 2.600 & CORE & primary analysis set \\
SY & 24 & 2.971 & 0.294 & -1.200 & 1.900 & excluded & prompt-format confound (12 A/B pairs; rigid VERDICT: vs reasoned commitment worth \textasciitilde +0.65..+0.94 in every condition including classical) \\
LC & 10 & 3.597 & -0.180 & -1.667 & 0.522 & excluded & harness-pathology contamination (LC-02 condition-independent parser failure; LC-03 drives 9/15 runaway timeouts; pubmed + failure mechanism identical across conditions) \\
XL & 8 & 3.390 & 0.632 & -0.800 & 1.925 & CORE & primary analysis set \\
SX & 6 & 3.068 & 1.701 & 1.075 & 2.333 & excluded & same silent-vs-explicit A/B wording confound as SY, already known \\
CB & 3 & 4.234 & 0.090 & -0.333 & 0.311 & CORE & primary analysis set \\
ES & 3 & 4.054 & 0.644 & -0.600 & 1.711 & CORE & primary analysis set \\
EN & 3 & 4.296 & 0.241 & -0.111 & 0.533 & CORE & primary analysis set \\
EB & 3 & 3.931 & 0.375 & -0.300 & 1.225 & CORE & primary analysis set \\
ZT & 2 & 4.936 & 0.050 & 0.000 & 0.100 & excluded & ceiling / zero discriminating power (4.90-5.00 every condition; manipulation check, not a comparison) \\
\bottomrule
\end{tabular}
\end{table}


==> tables_v2/T3_primary_result.tex <==
\begin{table}[t]
\centering
\caption{Primary question-level paired analysis. Per-question deltas of mean holistic score (condition $-$ classical); BCa 95\% CI from 10{,}000 question resamples; paired $t$, Wilcoxon signed-rank, and 10{,}000-flip sign-permutation $p$; paired $d_z$ and Cliff's $\delta$. Reported on CORE (34 questions) and all 76.}
\label{tab:primary_result}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
scope & contrast & n & mean\_delta & ci95 & t & df & p\_t & p\_wilcoxon & p\_perm & d\_z & cliffs\_delta & cliffs\_ci95 \\
\midrule
CORE & brainlm\_only - classical & 34 & 0.660 & [0.42, 0.92] & 5.000 & 33 & <0.001 & <0.001 & <0.001 & 0.860 & 0.443 & [0.18, 0.67] \\
CORE & omni\_only - classical & 34 & 0.442 & [0.22, 0.68] & 3.710 & 33 & <0.001 & 0.001 & <0.001 & 0.640 & 0.307 & [0.03, 0.56] \\
CORE & full - classical & 34 & 0.695 & [0.44, 0.97] & 5.020 & 33 & <0.001 & <0.001 & <0.001 & 0.860 & 0.473 & [0.22, 0.71] \\
CORE & anyFM - classical & 34 & 0.599 & [0.39, 0.82] & 5.380 & 33 & <0.001 & <0.001 & <0.001 & 0.920 & 0.407 & [0.15, 0.65] \\
all-76 & brainlm\_only - classical & 76 & 0.432 & [0.25, 0.62] & 4.450 & 75 & <0.001 & <0.001 & <0.001 & 0.510 & 0.262 & [0.08, 0.44] \\
all-76 & omni\_only - classical & 76 & 0.343 & [0.18, 0.52] & 3.880 & 75 & <0.001 & <0.001 & <0.001 & 0.450 & 0.208 & [0.03, 0.38] \\
all-76 & full - classical & 76 & 0.516 & [0.32, 0.72] & 5.010 & 75 & <0.001 & <0.001 & <0.001 & 0.580 & 0.305 & [0.12, 0.47] \\
all-76 & anyFM - classical & 76 & 0.431 & [0.27, 0.60] & 4.950 & 75 & <0.001 & <0.001 & <0.001 & 0.570 & 0.264 & [0.08, 0.44] \\
\bottomrule
\end{tabular}
\end{table}


==> tables_v2/T4_per_criterion.tex <==
\begin{table}[t]
\centering
\caption{Per-criterion paired effect (full $-$ classical, CORE, question-level). Raw $p$ from paired $t$; $q$ = Benjamini--Hochberg FDR across the 10 rubric fields; verdict at $q<0.05$. Ordered by effect size.}
\label{tab:per_criterion}
\begin{tabular}{lrrrrrr}
\toprule
criterion & tool\_facing & mean\_delta & d\_z & p & q\_BH & FDR\_verdict \\
\midrule
tool\_selection & yes & 1.088 & 1.290 & <0.001 & <0.001 & sig \\
information\_sufficiency & yes & 0.847 & 0.960 & <0.001 & <0.001 & sig \\
parameter\_validity & yes & 0.810 & 0.820 & <0.001 & <0.001 & sig \\
holistic\_score & no & 0.695 & 0.860 & <0.001 & <0.001 & sig \\
measurement\_grounding & yes & 0.666 & 0.820 & <0.001 & <0.001 & sig \\
reasoning\_coherence & no & 0.568 & 0.770 & <0.001 & <0.001 & sig \\
step\_level\_reasoning & no & 0.560 & 0.740 & <0.001 & <0.001 & sig \\
neural\_correlate\_consistency & no & 0.516 & 0.790 & <0.001 & <0.001 & sig \\
primitive\_fidelity & no & 0.244 & 0.310 & 0.077 & 0.077 & n.s. \\
epistemic\_calibration & no & 0.221 & 0.320 & 0.068 & 0.075 & n.s. \\
\bottomrule
\end{tabular}
\end{table}


==> tables_v2/T7_mixed_model.tex <==
\begin{table}[H]
\centering
\caption{Mixed-effects model \texttt{holistic\_score \textasciitilde{} C(cond) + (1|qid)} on run-level data, with the naive iid vs qid-clustered SE for the full-vs-classical effect and the resulting variance inflation factor.}
\label{tab:mixed_model}
\begin{tabular}{lrrrr}
\toprule
scope & term & coef & se & p \\
\midrule
CORE & Intercept & 3.224 & 0.108 & 0.000 \\
CORE & C(cond, Treatment('classical'))[T.brainlm\_only] & 0.658 & 0.070 & 0.000 \\
CORE & C(cond, Treatment('classical'))[T.omni\_only] & 0.449 & 0.070 & 0.000 \\
CORE & C(cond, Treatment('classical'))[T.full] & 0.696 & 0.071 & 0.000 \\
CORE & [full] OLS iid SE &  & 0.083 &  \\
CORE & [full] cluster(qid) SE &  & 0.140 &  \\
CORE & [full] variance inflation factor & 2.863 &  &  \\
CORE & ICC (question-level var / total) & 0.283 &  &  \\
all76 & Intercept & 3.109 & 0.086 & 0.000 \\
all76 & C(cond, Treatment('classical'))[T.brainlm\_only] & 0.426 & 0.048 & 0.000 \\
all76 & C(cond, Treatment('classical'))[T.omni\_only] & 0.342 & 0.048 & 0.000 \\
all76 & C(cond, Treatment('classical'))[T.full] & 0.514 & 0.048 & 0.000 \\
all76 & [full] OLS iid SE &  & 0.060 &  \\
all76 & [full] cluster(qid) SE &  & 0.102 &  \\
all76 & [full] variance inflation factor & 2.872 &  &  \\
all76 & ICC (question-level var / total) & 0.364 &  &  \\
\bottomrule
\end{tabular}
\end{table}


==> tables_v2/T8_directedness.tex <==
\begin{table}[t]
\centering
\caption{Question-directedness audit. Questions are tagged by which foundation model their
text names. The head-to-head gap is carried entirely by prompts that name BrainLM's tools --
which an \texttt{omni\_only} agent cannot call. On symmetric questions the gap is not
detectable. The single Omni-directed question runs the other way ($-1.40$).}
\label{tab:directedness}
\begin{tabular}{lrrrr}
\toprule
question subset & n & brainlm$-$omni & 95\% CI & $p$ \\
\midrule
brainlm-directed & 10 & +0.677 & [+0.34, +1.29] & 0.007 \\
symmetric & 20 & +0.151 & [-0.17, +0.51] & 0.398 \\
omni-directed & 1 & -1.400 & -- & -- \\
ALL CORE & 34 & +0.218 & [-0.03, +0.52] & 0.136 \\
\bottomrule
\end{tabular}
\end{table}

